Collaborative Multi-Robot Systems for Search and Rescue: Coordination and Perception

Autonomous or teleoperated robots have been playing increasingly important roles in civil applications in recent years. Across the different civil domains where robots can support human operators, one of the areas where they can have more impact is in search and rescue (SAR) operations. In particular, multi-robot systems have the potential to significantly improve the efficiency of SAR personnel with faster search of victims, initial assessment and mapping of the environment, real-time monitoring and surveillance of SAR operations, or establishing emergency communication networks, among other possibilities. SAR operations encompass a wide variety of environments and situations, and therefore heterogeneous and collaborative multi-robot systems can provide the most advantages. In this paper, we review and analyze the existing approaches to multi-robot SAR support, from an algorithmic perspective and putting an emphasis on the methods enabling collaboration among the robots as well as advanced perception through machine vision and multi-agent active perception. Furthermore, we put these algorithms in the context of the different challenges and constraints that various types of robots (ground, aerial, surface or underwater) encounter in different SAR environments (maritime, urban, wilderness or other post-disaster scenarios). This is, to the best of our knowledge, the first review considering heterogeneous SAR robots across different environments, while giving two complimentary points of view: control mechanisms and machine perception. Based on our review of the state-of-the-art, we discuss the main open research questions, and outline our insights on the current approaches that have potential to improve the real-world performance of multi-robot SAR systems.

==> authors.tex <==
%% Author Example:

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{a3.jpg}}]{Third C. Author, Jr.} (M'87) received the B.S. degree in mechanical 
% engineering from National Chung Cheng University, Chiayi, Taiwan, in 2004 
% and the M.S. degree in mechanical engineering from National Tsing Hua 
% University, Hsinchu, Taiwan, in 2006. He is currently pursuing the Ph.D. 
% degree in mechanical engineering at Texas A{\&}M University, College 
% Station, TX, USA.

% From 2008 to 2009, he was a Research Assistant with the Institute of 
% Physics, Academia Sinica, Tapei, Taiwan. His research interest includes the 
% development of surface processing and biological/medical treatment 
% techniques using nonthermal atmospheric pressure plasmas, fundamental study 
% of plasma sources, and fabrication of micro- or nanostructured surfaces. 

% Mr. Author's awards and honors include the Frew Fellowship (Australian 
% Academy of Science), the I. I. Rabi Prize (APS), the European Frequency and 
% Time Forum Award, the Carl Zeiss Research Award, the William F. Meggers 
% Award and the Adolph Lomb Medal (OSA).
% \end{IEEEbiography}
%----------------------------------------------------------------------------

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{people/jorge.jpg}}]{Jorge Peña Queralta} received B.S. degrees in mathematics and physics engineering from UPC BarcelonaTech, Spain, in 2016, a M.Sc. (Tech.) degree in Information and Communication Science and Technology from the University of Turku, Finland, and a M. Eng. degree in Electronics and Communication Engineering from Fudan University, China, in 2018. Since 2018, he has been a researcher and doctoral candidate at the Turku Intelligent Embedded and Robotic Systems Lab, University of Turku. His research interests include multi-robot systems, collaborative autonomy, swarm robotics, tand fog and edge computing.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{people/jussi_bw.jpg}}]{JUSSI TAIPALMAA} received BSc. degree in Signal Processing and Multimedia in 2013 and MSc. degree in Pervasive Systems in 2016, both from Tampere University of Technology. Since 2017, he has been a researcher and doctoral student in Signal Analysis and Machine Intelligence group in Tampere University. His research interests include machine learning, computer vision and biomedical signals along with software applications in autonomous and learning systems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{people/bilge-bw.jpg}}]{BILGE CAN PULLINEN} received her BSc. degree on Mechanical Engineering from Ege Universtiy, Izmir, Turkey in 2016. MSc. degree on Mechanical Design and Robot Engineering from Seoul National University of Science and Technology, Seoul, South Korea in 2019. Since early 2020, she has been a doctoral researcher at Doctoral Programme of Computing and Electrical Engineering in Signal Processing field at Tampere University. Her research interests include machine learning and computer vision.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{people/victor.jpg}}]{VICTOR KATHAN SARKER} (M'2017) 
received his BSc. degree on Electronic and Telecommunication Engineering from North South University, Dhaka, Bangladesh, in 2012 and MSc. (Tech.) degree on Embedded Computing from University of Turku, Finland, in 2017. From 2013 to 2015, he has worked as an Executive at the Department of Information Technology in Pacific Bangladesh Telecom Limited, Bangladesh. From 2016 to 2018, he worked as Research Assistant and Project Researcher in the iot4health research group at the Department of Information Technology, University of Turku, Finland. Since 2019, he has been working as a Researcher at the Department of Future Technologies in the same institution. His research interest includes IoT-based healthcare systems, IoE-based sensor nodes, safety and reliability of autonomous systems. He was awarded multiple government scholarships and several national awards from Science and Technology Weeks in Bangladesh. He received award of recognition from the Student Union of University of Turku, Finland, and works as the President of the TYY International Wing. He is a member of the IEEE Finland Section and acted as an Ambassador, IEEEXtreme 13.0 (Region 8). In leisure, he likes to sketch, sing, play instruments and volunteer.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{people/tuan.jpg}}]{TUAN NGUYEN GIA} PhD (Tech) is a senior researcher in Future Technologies Department, University of Turku. He has more than 50 international peer-reviewed articles and papers. He is an editor and topic editor of Vehicles and Sensors journal. He is also a reviewer of many journals such as IEEE Transactions of Industrial Informatics, IEEE Transactions of Mobile Computing and ACM Transactions Computing for Healthcare. His primary research interest is Internet of Things, Edge-AI and Fog computing. He is also interested in autonomous systems and reconfigurable computing with FPGA and CGRA.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{people/hannu.jpg}}]{HANNU TENHUNEN} is currently a Chair Professor of electronic systems with the Royal Institute of Technology (KTH), Stockholm, Sweden. He has held professor position as a Full Professor, an Invited Professor or a Visiting Honorary Professor in TUT, UTU, Finland, KTH, Sweden, Cornel U, USA, INPG, France, Fudan University, and Beijing Jiatong University, China, and The Chinese University of Hong Kong, Hong Kong. He has an Honorary Doctorate from the Tallinn University of Technology. He has served in the Technical Program Committees for all major conferences in his area. He has been a General Chairman or the Vice-Chairman or a member of the Steering Committee of multiple conferences in his core competence areas. He has been one of the founding editorial board members of three scientific journal, have been a Quest Editor of multiple special issues of scientific journals or books, and have contributed numerous invited articles to journals. He has contributed to over 850 international publications with H-index 47. He has nine international patents granted in multiple countries. He is also a member of the Academy of Engineering
Science of Finland
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{people/moncef.jpg}}]{Moncef Gabbouj} received the B.S. degree in electrical engineering from Oklahoma State University, Stillwater, OK, USA, in 1985, and the M.S. and Ph.D. degrees in electrical engineering from Purdue University, West Lafayette, IN, USA, in 1986 and 1989, respectively. He was an Academy of Finland Professor, from 2011 to 2015. He is currently a Professor of signal processing with the Faculty of Information Technology and Communication Sciences, Tampere University, Finland. He guided 40 Ph.D. students and published 650 papers. His current research interests include multimedia content-based analysis, indexing and retrieval, machine learning, nonlinear signal and image processing and analysis, voice conversion, and video processing and coding. Dr. Gabbouj is the past Chairman of the IEEE CAS TC on DSP and a Committee Member of the IEEE Fourier Award for Signal Processing. He served as an Associate Editor and a Guest Editor of many IEEE, and international journals and a Distinguished Lecturer for the IEEE CASS. He organized several tutorials and special sessions for major IEEE conferences and EUSIPCO. He is a member of the Academia Europaea and the Finnish Academy of Science and Letters.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{people/raitoharju2_1}}]{Jenni Raitoharju} received her Ph.D. degree at Tampere University of Technology, Finland in 2017. Since then, she has worked as a Postdoctoral Research Fellow at the Faculty of Information Technology and Communication Sciences, Tampere University, Finland. In 2019, she started working as a Senior Research Scientist at the Finnish Environment Institute, Jyväskylä, Finland after receiving Academy of Finland Postdoctoral Researcher funding for 2019-2022. She has co-authored 16 journal papers and 27 papers in international conferences. She is the chair of Young Academy Finland 2019-2020. Her research interests include machine learning and pattern recognition methods along with applications in biomonitoring and autonomous systems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{people/tomi.jpg}}]{Tomi Westerlund} is an Associate Professor of Autonomous Systems and Robotics at the University of Turku and a Research Professor at Wuxi Institute of Fudan University, Wuxi, China. Dr. Westerlund leads the Turku Intelligent Embedded and Robotic Systems research group (tiers.utu.fi), University of Turku, Finland. His current research interest is in the areas of Industrial IoT, smart cities and autonomous vehicles (aerial, ground and surface) as well as (co-)robots. In all these application areas, the core research interests are in multi-robot systems, collaborative sensing, interoperability, fog and edge computing, and edge AI.
\end{IEEEbiography}

==> sections/XX_OLD_TEXT.tex <==
%
%   ABSTRACT
%

%Use of automation has seen a rapid growth in recent years due to advancement in electronics, powerful embedded hardware with high computational capability and sophisticated software. Artificial intelligence, machine-learning and advanced algorithms embedded in the hardware have enabled airborne, surface and marine vehicles to perform tasks independently with very little human involvement. Development of multitude of sensors and energy-efficient electronics accompanying the automation is allowing researchers, engineers and developers across the world to collect several types of data for complex analysis and to perform application-specific tasks. Consequently, unmanned aerial vehicles (UAVs), especially drones are getting a lot of attention due to their versatile use in routine monitoring and Search and Rescue (SAR) operations, particularly during emergency situations. Swarm of drones can be deployed for this purpose for resource-efficient, self-governing and quicker response. Acting as the first-responder, this can significantly increase the chances of survival of the victims, especially in scenarios where human navigation is geographically challenging. However, designing such an autonomous system requires profound exploration in fields such as object detection, sensor fusion, inter-drone communication, swarm management, path planning and artificial intelligence. In this paper, we investigate these aspects, analyze the current state-of-the-art technology and provide a literature review of the current approaches when developing a SAR system incorporating autonomous multi-drone swarm. Furthermore, we also briefly discuss limitations and possible improvisation techniques where applicable.

%
%   SYSTEM
%


%\orange{Robotic SAR systems can differ in multiple ways: environment (land, sea), used equipment (USV, UAV, UGV), the level of autonomy, and the ways in which humans control the robotic systems. Factors such as complexity and density of SAR target environment, accessibility, span of the area where the SAR operation will take place affects the deployment requirements. For example, an accident in an urban area requires small number of autonomous drones but navigation and detection of victims is difficult. Schwoch et al. presented project IN-PREP, a simulation of a chemical leakage after a truck accident showing that a coordinated preparation for enhanced crisis management~\cite{schwochUnmanned2019}. In contrast, SAR in flooded rural area is comparatively simpler but can take a large fleet of drones.}

%\orange{SAR operations are mostly performed in times of need and when there is low chance of the subject to mitigate itself back to safety or normal situation. Depending on the weather condition, urgency, duration, span area of the search, geography, number of victims involved and surrounding environment the operation is to be performed in, unique approaches are required. We discuss few key points which are important to consider in such versatile SAR operational situations.}



% One crucial factor in aerial drones is the power source and for how long a drone can remain airborne. In a review, Boukoberine et al.~\cite{boukoberineDronePower2019} discussed currently used power supply architectures for drones and provided insights on their advantages and limitations. 





%A brief overview of wireless sensor and networking technologies for swarms of aquatic surface drones is provided in~\cite{velezWirelessSensor2016}. 






% weather condition-----------------
% One of the crucial factors which determines the success of autonomous SAR operation using is a favorable weather condition during it is performed. Complexity of the operation and level of human interaction in coordination of the SAR can elevate with bad weather condition and purpose-made hardware is needed~\cite{weatherVsDrones}. In~\cite{shamsiFoggyDrone2018}, the authors have presented a UAV for guiding the rescue vehicles to the incident site in foggy weather conditions. In addition, cold temperature depletes the battery capacity and fog/haze reduces areal visibility resulting in a shorter and more difficult navigation and detection, respectively. Besides, unstructured outdoor environment requires robust flight control for effective SAR operation. Maciel-Pearson et al.~\cite{pearsonMultitaskUAV2019} presented a multi-task regression-based learning for autonomous UAV flight control for such environments. Furthermore, in marine, especially at offshore, efficiency of SAR operations can dramatically change depending on wave levels. Takana et al.~\cite{takanaWaveAlert2018} provided a wave motion alert system using multiple drones and utilizing neural networks.

% urgency---------------------------
% SAR planning can be formed based on two-fold urgency aspect: the time period between the need of a SAR operation is recognized and the time the distress alert was received, and, how much time is in hand to execute the operation after receiving the distress alert. For example, if some hikers are missing in a forest area for 7 days and they could only convey an SOS message a day ago, or if there is a fire, the time in hand to react is short. In contrast, if people are stuck in a remote area with few days of food supply, this translates to more time for organized autonomous operation and narrowing down of search area by gathering as much information as possible. In~\cite{kratzkeOptimalPlanning2010}, an optimal planning approach SAROPS is presented for pre, during and post-distress periods.

% geography-------------------------
% The SAR target area can be classified into different types based on geographical state and thus requires specialized operation plan and autonomous robots/drones.









%\orange{In 2020, police and law enforcement agencies from several countries have used semi-autonomous fleets of areal drones over large areas to observe social distancing in order to minimize the spread of the COVID-19 virus. In addition, autonomous cargo drones have been deployed for delivery of food, test kits and emergency supply materials and kits during the exceptional pandemic circumstance \cite{delivery_drones_covid19}.}














% In~\cite{yongForestVision2018}, the authors have shown human object detection in the forest based on deep learning and drone vision.

% In~\cite{wangVortexSearch2018}, an optimal path planning method is presented based on adaptive vortex search algorithm for forest fire rescue.

% In~\cite{macwanMultirobot2015}, the authors presented a path-planning strategy for autonomous wilderness SAR.

% Similarly, in~\cite{zhilenkovForest2018}, a neural network and onboard parallel processing based autonomous system is developed for safely navigating in complex forest trails.

% For a different type of usage, Yoo et al. proposed a drone for detecting and understand the characteristics of the landmines~\cite{yooLandmineDetector2020}.




















% \begin{itemize}
%     \item The presence of hazardous materials, radiation areas, or high temperatures.
%     \item Localization and mapping of unknown, unstructured, dense and hazardous environments that result from disasters such as earthquakes or explosions, and in which robots are meant to operate.
%     \item Navigation in narrow spaces and uneven terrain, being able to traverse small apertures and navigate over unstable debris.
%     \item Close cooperation with human operators in a potentially shared operation space, requiring for well define human-robot interaction models.
% \end{itemize}

%The main benefits of involving autonomous robots in USAR scenarios are clear, including first and foremost to increase the safety of rescue personnel by reducing their exposure to potential hazards in the site and providing an initial assessment of the situation. The literature describes other potential opportunities of USAR robotics in terms of:
% \begin{itemize}
%     \item Relieving human personnel from emotional stress 
%     \item Reducing the time for locating survivors. Mortality in USAR scenarios raises significantly.
%     \item Assessing the structural parameters of the site and assist on remote triage.
%     \item Detecting and locating survivors and analyzing the surrounding structures.
%     \item Establishing a communication link to survivors.
% \end{itemize}



















% \orange{\textit{Some examples:
% 1: A drone may be completely human controlled.
% 2: A drone may do autonomous path planning and area coverage, but a human operator is monitoring the screen all the time.
% 3: A drone marks the interesting parts in the video, which a human operator needs to check.
% 4: The system is completely autonomous, it recognizes the victims and sends help in correct order.}}

%
%   Problem formulations
%

% \subsection{Optimization Objectives and Model Formulation} \red{TO DO}

% When considering the formulation of mission optimization objectives, multi-robot cooperation and perception models, and human-robot interaction methods, some of the most common approaches in SAR missions are the following:
% \red{TO DO}
% \begin{itemize}
%     \item \textbf{Search}
%     \item \textbf{Path Optimization}
%     \item \textbf{Fuel/Power Planning}
% \end{itemize}

% Graf et al. proposed an interesting approach for optimizing SAR vehicle path using ant colony system~\cite{grafAntColonySAR2017}.

%
%   POST-DISASTER SAR
%

% \paragraph{Natural calamities / Post-disaster SAR}

% Robots have the potential to support SAR operations in post-disaster scenarios. The literature includes examples of robotic systems being employed after natural calamities including earthquakes~\cite{nazarova2020application}, 

% % Earthquake, Hurricane, Flood, Wild-fire
% The potential of autonomous SAR is observed during and after natural calamities such as earthquake, hurricanes, floods and wild-fire. Particularly, the significant change in geographic accessibility (e.g. collapsed bridges, flooded roads due to an earthquake), managerial and coordination in crisis make the role of areal autonomous drones undeniably useful. Myeong et al. shows FAROS, a fireproof drone for SAR~\cite{myeongFireproofDrone2017}. Robust navigation, accurate vision and long operation time is required since the spread of affected area is often large and architectural damage (e.g. scattered debris and uprooted trees) makes search operations strenuous.  

% In a different work~\cite{huUAVhurricane2019}, a design approach for UAV-based disaster response in hurricane based on Euler cycle and integer programming is conferred.

% In~\cite{SAR-2007}, a description of an urban SAR scenario after an earthquake is provided.


%
%   COMMUNICATION
%

%For achieving a predefined target and completing an assigned task, robots in a multi-robots system communicate with their teammates to share their acquired information or future intentions. However, communication in multi-robot systems is challenging especially in harsh environments such as windy weather, storm, or areas lacking of network infrastructure.

%For instance, the packet loss rates increase dramatically when robots go beyond their communication ranges. In order to enhance communication's robustness and quality of service in multi-robot systems, two main areas including communication reliability and bandwidth utilization are focused. For improving communication reliability, main areas such as spatial estimation of communication reliability, guaranteeing connectivity through coordination, delay and disruption tolerant networking are often researched. To utilize bandwidth efficiently, communication decision making is investigated \cite{marcotte2019adaptive}.  

%Different communication methods such as \orange{short-range direct link based on 2.4~GHz ISM band, terrestrial, Wi-MAX, 4G LTE, and 5G  list...} have been proposed for inter-drone and drone-base data exchange and localization.

%Since drones roam in a three-dimensional space with complex environment around them, communication performance can vary due to interference, spatial scattering and wireless connectivity in a line-of-site (LOS) and non-LOS circumstances. Lye \textit{et al.} presented a novel 3D system model with detailed simulation showing effects on coverage \cite{lyuNetworkUAV3D2019} and investigating the challenges when incorporating existing cellular uplink/downlink channels for UAVs. 

%Zeng \textit{et al.} performed an meticulous study on UAV communication for incorporating upcoming cellular 5G communication and UAV-assisted wireless communication \cite{zengAccessSky5G2019}. The authors discussed UAV-ground aerial-terrestrial interference, quality of service (QoS) of payload data versus control information, resource limitation and difficulties introduced in communication due to high level of mobility. In a different work, Jawhar \textit{et al.} has presented a detailed classification and architectural review on existing communication and networking technologies used in UAV-based systems \cite{jawharUAVClassification2017}. Similarly, Yanmaz \textit{et al.} provided an overview of drone networks emphasizing on communication, coordination and sensing.

%L. Zeng \textit{et al.} has proposed a 3D Geometry-based Stochastic Channel Model for multi-input multi-output (MIMO) communication among UAVs \cite{zeng3DGBSM2017}. The authors investigated space-time correlation functions while navigating in a 3D environment and demonstrated that the direction of movement and location of the drones have significant impact for a sustained communication link. In addition, they also showed that horizontal drone movement achieves reliable MIMO performance.

%\subsection{Legislation}



\section{Communication}\label{sec:communication}

\red{Here we probably need help from someone, who is more proficient in communications technology. Now the division is done quite roughly.}

Different communication methods such as \orange{short-range direct link based on 2.4~GHz ISM band, terrestrial, Wi-MAX, 4G LTE, and 5G  list...} have been proposed for inter-drone and drone-base data exchange and localization.


\subsection{3D Environment}

Since drones roam in a three-dimensional space with complex environment around them, communication performance can vary due to interference, spatial scattering and wireless connectivity in a line-of-site (LOS) and non-LOS circumstances. Lye \textit{et al.} presented a novel 3D system model with detailed simulation showing effects on coverage \cite{lyuNetworkUAV3D2019} and investigating the challenges when incorporating existing cellular uplink/downlink channels for UAVs. 



\subsection{Mobility and Real-Time Data Exchange}

% FANET, VANET



\subsection{Connectivity and Network Topology}

Zeng \textit{et al.} performed an meticulous study on UAV communication for incorporating upcoming cellular 5G communication and UAV-assisted wireless communication \cite{zengAccessSky5G2019}. The authors discussed UAV-ground aerial-terrestrial interference, quality of service (QoS) of payload data versus control information, resource limitation and difficulties introduced in communication due to high level of mobility. In a different work, Jawhar \textit{et al.} has presented a detailed classification and architectural review on existing communication and networking technologies used in UAV-based systems \cite{jawharUAVClassification2017}. Similarly, Yanmaz \textit{et al.} provided an overview of drone networks emphasizing on communication, coordination and sensing \cite{}.




\subsubsection{Drone-to-Drone Communication (air-air)}



\subsubsection{Drone-to-Base Communication (ground-air)}




\subsection{Simultaneous Communication and Localization}

L. Zeng\textit{et al.} has proposed a 3D Geometry-based Stochastic Channel Model for multi-input multi-output (MIMO) communication among UAVs \cite{zeng3DGBSM2017}. The authors investigated space-time correlation functions while navigating in a 3D environment and demonstrated that the direction of movement and location of the drones have significant impact for a sustained communication link. In addition, they also showed that horizontal drone movement achieves reliable MIMO performance.





\subsection{Reliability and Synchronization}
% Primary link

% Secondary High bandwidth link (for U/HD data transfer)

% Backup link




\subsection{Scalability}



\section{Conclusion}\label{sec:conclusion}

Embedded systems combined with sophisticated electronics and efficient software algorithms have pushed the boundary further to make automation based on artificial intelligence possible. Autonomous airborne, surface and marine vehicles can now take these into use for various time and effort-wise costly purposes such as SAR operations. Besides routine monitoring and observation, such a system can be particularly important in post-disaster situations acting as fastest responder to the scene. In this paper, we have taken a detailed look on autonomous multi-robot SAR operations keeping our focus on strategic collaboration, efficient software algorithms and real-time machine learning models which enables robust sensor fusion. We have classified previously performed research and works according to decision making approach, distributed role assignment, dynamic task management. In addition, we have also analyzed and discussed active vision approaches based on machine learning. Furthermore, we have inspected independent and cooperative modes of operation for autonomous vehicles used in SAR application scenario.

==> sections/XX_Resources.tex <==
\section{Resources for the paper: (Will be removed)}

\blue{Please use this section for gathering any interesting resource you may have found to keep the sections clean}

\begin{itemize}
    \item German Rescue Robotics Center at Fraunhofer FKIE \href{https://www.fkie.fraunhofer.de/en/press-releases/a-drz_project_launch.html}{New center of excellence to drive innovation in rescue robots}
    \item One potential source of material is the IEEE International Symposium on Safety, Security, and Rescue Robotics (SSRR).
    \item Another one is projects from the European Robotics League Emergency Tournament
    \item Also EU projects: NIFTi, ICARUS, TRADR, CENTAURO, SmokeBot
\end{itemize}

